Constrained Assortment Optimization under the Cross-Nested Logit Model

We study the assortment optimization problem under general linear constraints, where the customer choice behavior is captured by the Cross-Nested Logit model. In this problem, there is a set of products organized into multiple subsets (or nests), where each product can belong to more than one nest. The aim is to find an assortment to offer to customers so that the expected revenue is maximized. We show that, under the Cross-Nested Logit model, the assortment problem is NP-hard, even without any constraints. To tackle the assortment optimization problem, we develop a new discretization mechanism to approximate the problem by a linear fractional program with a performance guarantee of $\frac{1 - \epsilon}{1+\epsilon}$, for any accuracy level $\epsilon>0$. We then show that optimal solutions to the approximate problem can be obtained by solving mixed-integer linear programs. We further show that our discretization approach can also be applied to solve a joint assortment optimization and pricing problem, as well as an assortment problem under a mixture of Cross-Nested Logit models to account for multiple classes of customers. Our empirical results on a large number of randomly generated test instances demonstrate that, under a performance guarantee of 90%, the percentage gaps between the objective values obtained from our approximation methods and the optimal expected revenues are no larger than 1.2%.

==> tables/assortment_large_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}
\centering
\caption{Results on the large dataset of the assortment with $\epsilon = 5e-2$. The symbol "-" indicates that the solver exceeds the time budget.}
\label{table:assortment_large}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}ccllllllllllll@{}}
\toprule
\multirow{3}{*}{m} & \multirow{3}{*}{N} &  & \multicolumn{2}{c}{\multirow{2}{*}{\# (Solved instances)}} &  & \multicolumn{2}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\# (Instances with \\      best objective)\end{tabular}}} &  & \multicolumn{2}{l}{\multirow{2}{*}{Average gap (\%)}} &  & \multicolumn{2}{l}{\multirow{2}{*}{Computing time (s)}} \\
                   &                    &  & \multicolumn{2}{c}{}                                       &  & \multicolumn{2}{l}{}                                                                                                    &  & \multicolumn{2}{l}{}                                  &  & \multicolumn{2}{l}{}                                    \\ \cmidrule(lr){4-5} \cmidrule(lr){7-8} \cmidrule(lr){10-11} \cmidrule(l){13-14} 
                   &                    &  & Bisection                        & MILP                    &  & Bisection                                                       & MILP                                                  &  & Bisection                     & MILP                  &  & Bisection                        & MILP                 \\ \midrule
200                & 5                  &  & \textbf{10}                      & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 28.43                 &  & \textbf{26.61}                   & -                    \\
200                & 10                 &  & \textbf{10}                      & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 22.36                 &  & \textbf{73.00}                   & -                    \\
300                & 5                  &  & \textbf{10}                      & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 42.15                 &  & \textbf{80.38}                   & -                    \\
300                & 10                 &  & \textbf{10}                      & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 38.91                 &  & \textbf{265.90}                  & -                    \\
400                & 5                  &  & \textbf{10}                      & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 46.80                 &  & \textbf{203.11}                  & -                    \\
400                & 10                 &  & \textbf{9}                       & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 40.47                 &  & \textbf{439.70}                  & -                    \\
500                & 5                  &  & \textbf{10}                      & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 43.22                 &  & \textbf{553.95}                  & -                    \\
500                & 10                 &  & \textbf{8}                       & 0                       &  & \textbf{10}                                                     & 0                                                     &  & \textbf{0.00}                 & 64.44                 &  & \textbf{1145.10}                 & -                    \\ \midrule
\multicolumn{2}{c}{Total}             &  & \textbf{77}                     & 0.0                     &  & \textbf{80}                                                   & 0.0                                                   &  & \textbf{0.00}                 & 40.85                 &  & \textbf{348.47}                  & -                    \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/assortment_small.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}
\centering
\caption{Results on the small dataset of assortment problem with approximation error $\epsilon = 1e-1$.}
\label{table:sensitivity}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{ccllllllllllll}
\hline
\multirow{2}{*}{N} & \multirow{2}{*}{m} &  & \multicolumn{3}{l}{\#   Solved instances}     &  & \multicolumn{3}{l}{Average   computing time (s)} &  & \multicolumn{3}{l}{Average   gap (\%)} \\ \cline{4-6} \cline{8-10} \cline{12-14} 
                   &                    &  & Bisection      & MILP           & SOCP        &  & Bisection        & MILP             & SOCP       &  & Bisection        & MILP     & SOCP     \\ \hline
5                  & 20                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 0.34             & \textbf{0.05}    & 4.50       &  & \textbf{0.00}    & 29.12    & 98.61    \\
5                  & 30                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 0.62             & \textbf{0.14}    & 7.10       &  & \textbf{0.00}    & 30.54    & 65.49    \\
5                  & 40                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 0.91             & \textbf{0.19}    & 46.70      &  & \textbf{0.00}    & 21.58    & 52.62    \\
5                  & 50                 &  & \textbf{10}    & \textbf{10}    & 9           &  & 1.45             & \textbf{0.34}    & 600.00     &  & \textbf{0.00}    & 20.27    & 51.30    \\
5                  & 60                 &  & \textbf{10}    & \textbf{10}    & 2           &  & 2.23             & \textbf{0.59}    & 1077.70    &  & \textbf{0.00}    & 20.79    & 36.63    \\
5                  & 70                 &  & \textbf{10}    & \textbf{10}    & 0           &  & 2.82             & \textbf{1.12}    & -          &  & \textbf{0.00}    & 24.68    & 25.09    \\
5                  & 80                 &  & \textbf{10}    & \textbf{10}    & 0           &  & 3.86             & \textbf{1.55}    & -          &  & \textbf{0.00}    & 14.95    & 35.16    \\
5                  & 90                 &  & \textbf{10}    & \textbf{10}    & 0           &  & 5.33             & \textbf{2.50}    & -          &  & \textbf{0.00}    & 31.15    & 34.34    \\
5                  & 100                &  & \textbf{10}    & \textbf{10}    & 0           &  & \textbf{7.03}    & 7.90             & -          &  & \textbf{0.00}    & 16.22    & 31.58    \\
10                 & 20                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 0.11             & \textbf{0.02}    & 1.01       &  & \textbf{0.56}    & 18.06    & 388.57   \\
10                 & 30                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 0.40             & \textbf{0.06}    & 4.96       &  & \textbf{0.00}    & 28.87    & 452.05   \\
10                 & 40                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 1.16             & \textbf{0.12}    & 12.15      &  & \textbf{0.00}    & 25.67    & 159.47   \\
10                 & 50                 &  & \textbf{10}    & \textbf{10}    & \textbf{10} &  & 1.58             & \textbf{0.19}    & 192.86     &  & \textbf{0.00}    & 31.92    & 88.67    \\
10                 & 60                 &  & \textbf{10}    & \textbf{10}    & 8           &  & 2.03             & \textbf{0.33}    & 834.81     &  & \textbf{0.00}    & 26.85    & 61.87    \\
10                 & 70                 &  & \textbf{10}    & \textbf{10}    & 1           &  & 3.42             & \textbf{0.57}    & 2362.27    &  & \textbf{0.00}    & 28.92    & 54.55    \\
10                 & 80                 &  & \textbf{10}    & \textbf{10}    & 0           &  & 4.42             & \textbf{0.88}    & -          &  & \textbf{0.00}    & 32.06    & 60.32    \\
10                 & 90                 &  & \textbf{10}    & \textbf{10}    & 0           &  & 8.86             & \textbf{1.45}    & -          &  & \textbf{0.00}    & 26.30    & 49.89    \\
10                 & 100                &  & \textbf{10}    & \textbf{10}    & 0           &  & 13.72            & \textbf{3.37}    & -          &  & \textbf{0.00}    & 26.42    & 46.17    \\ \hline
\multicolumn{3}{l}{Average}                & \textbf{10.0} & \textbf{10.0} & 5.0        &  & 3.35             & \textbf{1.19}    & -          &  & \textbf{0.03}    & 25.24    & 99.58    \\ \hline
\end{tabular}}
\end{table}

==> tables/k_milp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\caption{Number of sub-intervals generated for the mixed-integer linear program (section \ref{sec:milp})}
\label{tab:k_milp}
\begin{tabular}{@{}lllllllllllllllll@{}}
\toprule
$\sigma_n$          &  & 0.5 & 0.5 & 0.5 & 0.6 & 0.6 & 0.6 & 0.7 & 0.7 & 0.7 & 0.8 & 0.8 & 0.8 & 0.9 & 0.9 & 0.9 \\ \midrule
$U_n$             &  & 5   & 10  & 15  & 5   & 10  & 15  & 5   & 10  & 15  & 5   & 10  & 15  & 5   & 10  & 15  \\ \midrule
$\epsilon$ = 0.5  &  & 2   & 3   & 4   & 2   & 3   & 3   & 2   & 3   & 3   & 2   & 3   & 4   & 3   & 3   & 4   \\
$\epsilon$ = 0.1  &  & 9   & 13  & 15  & 10  & 14  & 16  & 11  & 16  & 18  & 13  & 18  & 21  & 14  & 20  & 24  \\
$\epsilon$ = 0.05 &  & 17  & 24  & 28  & 19  & 27  & 32  & 22  & 32  & 37  & 26  & 36  & 43  & 29  & 41  & 48  \\
$\epsilon$ = 0.01 &  & 81  & 116 & 137 & 97  & 138 & 162 & 113 & 161 & 189 & 129 & 184 & 216 & 145 & 207 & 243 \\ \bottomrule
\end{tabular}
\end{table}
